Knowledge from Probability

We give a probabilistic analysis of inductive knowledge and belief and explore its predictions concerning knowledge about the future, about laws of nature, and about the values of inexactly measured quantities. The analysis combines a theory of knowledge and belief formulated in terms of relations of comparative normality with a probabilistic reduction of those relations. It predicts that only highly probable propositions are believed, and that many widely held principles of belief-revision fail.

==> eptcsdata.tex <==
\providecommand{\firstpage}{171}
\providecommand{\publicationstatus}{J. Y. Halpern and A. Perea (Eds.): Theoretical Aspects \\
of Rationality and Knowledge 2021 (TARK 2021) \\
EPTCS 335, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.335.15}{10.4204/EPTCS.335.15}}
\pdfoutput=1

